Intent-conditioned and Non-toxic Counterspeech Generation using Multi-Task Instruction Tuning with RLAIF

Counterspeech, defined as a response to mitigate online hate speech, is increasingly used as a non-censorial solution. Addressing hate speech effectively involves dispelling the stereotypes, prejudices, and biases often subtly implied in brief, single-sentence statements or abuses. These implicit expressions challenge language models, especially in seq2seq tasks, as model performance typically excels with longer contexts. Our study introduces CoARL, a novel framework enhancing counterspeech generation by modeling the pragmatic implications underlying social biases in hateful statements. CoARL's first two phases involve sequential multi-instruction tuning, teaching the model to understand intents, reactions, and harms of offensive statements, and then learning task-specific low-rank adapter weights for generating intent-conditioned counterspeech. The final phase uses reinforcement learning to fine-tune outputs for effectiveness and non-toxicity. CoARL outperforms existing benchmarks in intent-conditioned counterspeech generation, showing an average improvement of 3 points in intent-conformity and 4 points in argument-quality metrics. Extensive human evaluation supports CoARL's efficacy in generating superior and more context-appropriate responses compared to existing systems, including prominent LLMs like ChatGPT.

==> sections/error_analysis.tex <==
\section{Error Analysis \amey{TODO} \aswini{TODO}}


==> tables/table4.tex <==
\begin{table*}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Hate speech}} & \multicolumn{5}{c}{\textbf{Counter speech type}} \\ 
\midrule
\textbf{Target group} & \textbf{Count} & \textbf{INF} & \textbf{POS} & \textbf{QUE} & \textbf{DEN} & \textbf{Total} \\ 
\midrule
\textbf{Muslims} & 914 & 914 & 914 & 914 & 914 & 3656 \\
\textbf{Women} & 508 & 508 & 508 & 508 & 508 & 2032 \\
\textbf{LGBTQ+} & 449 & 449 & 449 & 449 & 449 & 1796 \\
\textbf{Jews} & 392 & 392 & 392 & 392 & 392 & 1568 \\
\textbf{Refugees} & 70 & 70 & 70 & 70 & 70 & 280 \\
\textbf{Asian people} & 29 & 29 & 29 & 29 & 29 & 116 \\
\textbf{Immigrants} & 562 & 562 & 562 & 562 & 562 & 2248 \\
\textbf{PwD} & 173 & 173 & 173 & 173 & 173 & 304 \\
\textbf{POC} & 306 & 306 & 306 & 306 & 306 & 80 \\
\textbf{Other} & 85 & 85 & 85 & 85 & 85 & 208 \\
\midrule
\textbf{Total} & 3488 & 3488 & 3488 & 3488 & 3488 & 13952 \\
\textbf{Train} & 2383 & 2383 & 2383 & 2383 & 2383 & 9532 \\
\textbf{Validation} & 365 & 365 & 365 & 365 & 365 & 1460 \\
\textbf{Test} & 740 & 740 & 740 & 740 & 740 & 2960 \\
\bottomrule
\end{tabular}%
}
\end{center}
\caption{Statistics of IntentCONAN 2.0}
\label{tab:table_1}
\end{table*}

